Energy-efficient localised rollback after failures via data flow analysis

Exascale systems will suffer failures hourly. HPC programmers rely mostly on application-level checkpoint and a global rollback to recover. In recent years, techniques reducing the number of rolling back processes have been implemented via message logging. However, the log-based approaches have weaknesses, such as being dependent on complex modifications within an MPI implementation, and the fact that a full restart may be required in the general case. To address the limitations of all log-based mechanisms, we return to checkpoint-only mechanisms, but advocate data-flow-driven recovery (DFR), a fundamentally different approach relying on analysis of the data flow of iterative codes, and the well-known concept of data-flow graphs. We demonstrate the effectiveness of DFR for an MPI stencil code to optimise rollback and reduce the overall energy consumption by 10-12 % on idling nodes during localised rollback. We also provide large-scale estimates for the energy savings of DFR compared to global rollback, which for stencil codes increase as n square for a process count n.

==> virtual-topology-2x4.tex <==
\begin{figure}

\begin{tikzpicture}
\newcounter{row}
\newcounter{col}
\newcommand\setrow[2]{
  \setcounter{col}{1}
  \foreach \n in {#1, #2} {
    \edef\x{\value{col} - 0.5}
    \edef\y{4.5 - \value{row}}
    \node[anchor=center] at (\x, \y) {\n};
    \stepcounter{col}
  }
  \stepcounter{row}
}
    \draw (0, 0) grid (2, 4);
  \setcounter{row}{1}
   \setrow {13}{13}
   \setrow {13}{13}
   \setrow {13}{13}
   \setrow {13}{\color{red}13}
   
   
        
  \begin{scope}[xshift=5cm]
     \draw (0, 0) grid (2,4);
  \setcounter{row}{1}
   \setrow {10(0)}{10(0)}{10(0)}{10(0)}
   \setrow {\color{pink}10(3)}{\color{pink}11(3)}%{\color{pink}10(3)}{\color{pink}10(3)}
   \setrow {\color{pink}10(3)}{\color{pink}10(3)}%{\color{pink}10(3)}{\color{pink}10(3)}
   \setrow {\color{pink}10(3)}{\color{red}10(3)}%{\color{pink}10(3)}{\color{pink}10(3)} 
   
   \draw[very thick] (0,0) -- (2, 0) -- (2,1) -- (0,1) -- (0,0);
\draw[very thick] (0,1) -- (2, 1) -- (2,2) -- (0,2) -- (0,1);
\draw[very thick] (0,2) -- (2, 2) -- (2,3) -- (0,3) -- (0,2);
\draw[very thick] (0,3) -- (2, 3) -- (2,4) -- (0,4) -- (0,3);

  \end{scope}  

\draw[very thick] (0,0) -- (2, 0) -- (2,1) -- (0,1) -- (0,0);
\draw[very thick] (0,1) -- (2, 1) -- (2,2) -- (0,2) -- (0,1);
\draw[very thick] (0,2) -- (2, 2) -- (2,3) -- (0,3) -- (0,2);
\draw[very thick] (0,3) -- (2, 3) -- (2,4) -- (0,4) -- (0,3);

\node[rectangle] (a) at (4.5,0.5) {node1};
\node[rectangle] (a) at (4.5,1.5) {node2};
\node[rectangle] (a) at (4.5,2.5) {node3};
\node[rectangle] (a) at (4.5,3.5) {node4};

 \end{tikzpicture}
\caption{Outline of completed iterations per process in the described 2D topology. Left: Global rollback iterations. Right: Non-global rollback iterations, with numbers in brackets indicating how many iterations are done by process to support replacement process; Failed/replacement process marked in red.}
\label{setting1}
\end{figure}

